The LiteBIRD mission to explore cosmic inflation

LiteBIRD, the next-generation cosmic microwave background (CMB) experiment, aims for a launch in Japan's fiscal year 2032, marking a major advancement in the exploration of primordial cosmology and fundamental physics. Orbiting the Sun-Earth Lagrangian point L2, this JAXA-led strategic L-class mission will conduct a comprehensive mapping of the CMB polarization across the entire sky. During its 3-year mission, LiteBIRD will employ three telescopes within 15 unique frequency bands (ranging from 34 through 448 GHz), targeting a sensitivity of 2.2\,$\mu$K-arcmin and a resolution of 0.5$^\circ$ at 100\,GHz. Its primary goal is to measure the tensor-to-scalar ratio $r$ with an uncertainty $\delta r = 0.001$, including systematic errors and margin. If $r \geq 0.01$, LiteBIRD expects to achieve a $>5\sigma$ detection in the $\ell=$2-10 and $\ell=$11-200 ranges separately, providing crucial insight into the early Universe. We describe LiteBIRD's scientific objectives, the application of systems engineering to mission requirements, the anticipated scientific impact, and the operations and scanning strategies vital to minimizing systematic effects. We will also highlight LiteBIRD's synergies with concurrent CMB projects.

==> authors_affiliations_LB_2024.05_general_spie.tex <==
% Ensure the `authblk` package is loaded:
\makeatletter
\@ifpackageloaded{authblk}{}{%
    \@ifpackageloaded{authblk-TI}{}{%
        \usepackage{authblk}% allows handling of the `_authblk.tex` file
    }%
}%
\makeatother

% The following lines handle the prepending/appending of "LiteBIRD Collaboration" for key/general/special papers:
\makeatletter
\def\@author{}
\renewcommand\@author{%
    \ifx\AB@affillist\AB@empty%
        \AB@author%
    \else%
        \ifnum\value{affil}>\value{Maxaffil}%
            \def\rlap##1{##1} \AB@authlist \\LiteBIRD Collaboration.\\[\affilsep]\AB@affillist%
        \else%
            \AB@authors%
        \fi%
    \fi%
}
\makeatother

% Uncomment the following lines if you want to customize the author and affiliation fonts.
% For font types you can use: normalfont, bfseries, itshape, scshape.
% For font sizes you can use: tiny, scriptsize, footnotesize, small, normalsize, large, Large.
\renewcommand\Authfont{\normalfont\normalsize}  % normal sized normal font
\renewcommand\Affilfont{\itshape\small}         % small  sized italic font

\author[1]{T.\,Ghigna}
\author[2]{A.\,Adler}
\author[3]{K.\,Aizawa}
\author[1]{H.\,Akamatsu}
\author[3]{R.\,Akizawa}
\author[4]{E.\,Allys}
\author[5]{A.\,Anand}
\author[6]{J.\,Aumont}
\author[7]{J.\,Austermann}
\author[8]{S.\,Azzoni}
\author[9,10,11]{C.\,Baccigalupi}
\author[12,13,14]{M.\,Ballardini}
\author[6]{A.\,J.\,Banday}
\author[15]{R.\,B.\,Barreiro}
\author[16,17,18]{N.\,Bartolo}
\author[19]{S.\,Basak}
\author[20]{A.\,Basyrov}
\author[21]{S.\,Beckman}
\author[22,23]{M.\,Bersanelli}
\author[12,13]{M.\,Bortolami}
\author[24]{F.\,Bouchet}
\author[12]{T.\,Brinckmann}
\author[13,25,26]{P.\,Campeti}
\author[6]{E.\,Carinos}
\author[5,27]{A.\,Carones}
\author[15]{F.\,J.\,Casas}
\author[28,21,29,30]{K.\,Cheung}
\author[1,31]{Y.\,Chinone}
\author[32]{L.\,Clermont}
\author[33,34]{F.\,Columbro}
\author[33,34]{A.\,Coppolecchia}
\author[29]{D.\,Curtis}
\author[33,34]{P.\,de\,Bernardis}
\author[35,1]{T.\,de\,Haan}
\author[36,15,37]{E.\,de\,la\,Hoz}
\author[33,34]{M.\,De\,Petris}
\author[38]{S.\,Della\,Torre}
\author[39]{G.\,Delle\,Monache}
\author[40]{E.\,Di\,Giorgi}
\author[28]{C.\,Dickinson}
\author[25,37]{P.\,Diego-Palazuelos}
\author[41]{J.\,J.\,Díaz\,García}
\author[42]{M.\,Dobbs}
\author[43,44]{T.\,Dotani}
\author[33,34]{G.\,D’Alessandro}
\author[20]{H.\,K.\,Eriksen}
\author[45]{J.\,Errard}
\author[46]{T.\,Essinger-Hileman}
\author[47]{N.\,Farias}
\author[31]{E.\,Ferreira}
\author[22,23]{C.\,Franceschet}
\author[20]{U.\,Fuskeland}
\author[12,5]{G.\,Galloni}
\author[20]{M.\,Galloway}
\author[45]{K.\,Ganga}
\author[13]{M.\,Gerbino}
\author[48,38]{M.\,Gervasi}
\author[41,49]{R.\,T.\,Génova-Santos}
\author[50]{S.\,Giardiello}
\author[15]{C.\,Gimeno-Amo}
\author[20]{E.\,Gjerløw}
\author[41]{R.\,González\,González}
\author[45]{L.\,Grandsire}
\author[14,51]{A.\,Gruppuso}
\author[52]{N.\,W.\,Halverson}
\author[50]{P.\,Hargrave}
\author[28]{S.\,E.\,Harper}
\author[1,35,43,31,44]{M.\,Hazumi}
\author[53]{S.\,Henrot-Versillé}
\author[54]{L.\,T.\,Hergt}
\author[15]{D.\,Herranz}
\author[24]{E.\,Hivon}
\author[55]{R.\,A.\,Hlozek}
\author[56]{T.\,D.\,Hoang}
\author[7]{J.\,Hubmayr}
\author[57]{K.\,Ichiki}
\author[58]{K.\,Ikuma}
\author[58]{H.\,Ishino}
\author[7]{G.\,Jaehnig}
\author[31]{B.\,Jost}
\author[35]{K.\,Kohri}
\author[59]{K.\,Konishi}
\author[33,34]{L.\,Lamagna}
\author[13]{M.\,Lattanzi}
\author[31]{C.\,Leloup}
\author[4]{F.\,Levrier}
\author[5]{A.\,I.\,Lonappan}
\author[60]{G.\,Luzzi}
\author[61]{J.\,Macias-Perez}
\author[62]{B.\,Maffei}
\author[33]{E.\,Marchitelli}
\author[15]{E.\,Martínez-González}
\author[33,34]{S.\,Masi}
\author[16,17,18,63]{S.\,Matarrese}
\author[31]{T.\,Matsumura}
\author[33]{S.\,Micheli}
\author[5,27]{M.\,Migliaccio}
\author[25]{M.\,Monelli}
\author[6]{L.\,Montier}
\author[14]{G.\,Morgante}
\author[4,6]{L.\,Mousset}
\author[58]{Y.\,Nagano}
\author[43]{R.\,Nagata}
\author[12,13]{P.\,Natoli}
\author[33]{A.\,Novelli}
\author[50]{F.\,Noviello}
\author[31]{I.\,Obata}
\author[33]{A.\,Occhiuzzi}
\author[43]{K.\,Odagiri}
\author[58]{R.\,Omae}
\author[12,13,62]{L.\,Pagano}
\author[33,34]{A.\,Paiella}
\author[14,51]{D.\,Paoletti}
\author[15]{G.\,Pascual-Cisneros}
\author[45]{G.\,Patanchon}
\author[64,65]{V.\,Pavlidou}
\author[33,34]{F.\,Piacentini}
\author[45]{M.\,Piat}
\author[5]{G.\,Piccirilli}
\author[40]{M.\,Pinchera}
\author[33]{G.\,Pisano}
\author[39]{L.\,Porcelli}
\author[12]{N.\,Raffuzzi}
\author[21]{C.\,Raum}
\author[15,28]{M.\,Remazeilles}
\author[27,4]{A.\,Ritacco}
\author[41,49]{J.\,Rubino-Martin}
\author[15,37]{M.\,Ruiz-Granda}
\author[66,31]{Y.\,Sakurai}
\author[67]{G.\,Savini}
\author[54]{D.\,Scott}
\author[43,68]{Y.\,Sekimoto}
\author[66]{M.\,Shiraishi}
\author[69,40]{G.\,Signorelli}
\author[58,31]{S.\,L.\,Stever}
\author[54]{R.\,M.\,Sullivan}
\author[30]{A.\,Suzuki}
\author[3,43]{R.\,Takaku}
\author[43]{H.\,Takakura}
\author[31]{S.\,Takakura}
\author[58]{Y.\,Takase}
\author[40,69]{A.\,Tartari}
\author[64,65]{K.\,Tassis}
\author[70,71]{K.\,L.\,Thompson}
\author[22,23]{M.\,Tomasi}
\author[53]{M.\,Tristram}
\author[50]{C.\,Tucker}
\author[9]{L.\,Vacher}
\author[53]{B.\,van\,Tent}
\author[15]{P.\,Vielva}
\author[43]{K.\,Watanuki}
\author[20]{I.\,K.\,Wehus}
\author[21]{B.\,Westbrook}
\author[53]{G.\,Weymann-Despres}
\author[72,67]{B.\,Winter}
\author[46]{E.\,J.\,Wollack}
\author[73]{A.\,Zacchei}
\author[48,38]{M.\,Zannoni}
\author[1]{Y.\,Zhou}
\affil[1]{International Center for Quantum-field Measurement Systems for Studies of the Universe and Particles (QUP), High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki 305-0801, Japan}
\affil[2]{The Oskar Klein Centre, Department of Physics, Stockholm University, SE-106 91 Stockholm, Sweden}
\affil[3]{The University of Tokyo, Department of Physics, Tokyo 113-0033, Japan}
\affil[4]{Laboratoire de Physique de l’École Normale Supérieure, ENS, Université PSL, CNRS, Sorbonne Université, Université de Paris, 75005 Paris, France}
\affil[5]{Dipartimento di Fisica, Università di Roma Tor Vergata, Via della Ricerca Scientifica, 1, 00133, Roma, Italy}
\affil[6]{IRAP, Université de Toulouse, CNRS, CNES, UPS, Toulouse, France}
\affil[7]{NIST Quantum Sensors Group, 325 Broadway, Boulder, CO 80305, USA}
\affil[8]{Department of Astrophysical Sciences, Peyton Hall, Princeton University, Princeton, NJ, USA 08544}
\affil[9]{International School for Advanced Studies (SISSA), Via Bonomea 265, 34136, Trieste, Italy}
\affil[10]{INFN Sezione di Trieste, via Valerio 2, 34127 Trieste, Italy}
\affil[11]{IFPU, Via Beirut, 2, 34151 Grignano, Trieste, Italy}
\affil[12]{Dipartimento di Fisica e Scienze della Terra, Università di Ferrara, Via Saragat 1, 44122 Ferrara, Italy}
\affil[13]{INFN Sezione di Ferrara, Via Saragat 1, 44122 Ferrara, Italy}
\affil[14]{INAF - OAS Bologna, via Piero Gobetti, 93/3, 40129 Bologna, Italy}
\affil[15]{Instituto de Fisica de Cantabria (IFCA, CSIC-UC), Avenida los Castros SN, 39005, Santander, Spain}
\affil[16]{Dipartimento di Fisica e Astronomia “G. Galilei”, Università degli Studi di Padova, via Marzolo 8, I-35131 Padova, Italy}
\affil[17]{INFN Sezione di Padova, via Marzolo 8, I-35131, Padova, Italy}
\affil[18]{INAF, Osservatorio Astronomico di Padova, Vicolo dell’Osservatorio 5, I-35122, Padova, Italy}
\affil[19]{School of Physics, Indian Institute of Science Education and Research Thiruvananthapuram, Maruthamala PO, Vithura, Thiruvananthapuram 695551, Kerala, India}
\affil[20]{Institute of Theoretical Astrophysics, University of Oslo, Blindern, Oslo, Norway}
\affil[21]{University of California, Berkeley, Department of Physics, Berkeley, CA 94720, USA}
\affil[22]{Dipartimento di Fisica, Università degli Studi di Milano, Via Celoria 16 - 20133, Milano, Italy}
\affil[23]{INFN Sezione di Milano, Via Celoria 16 - 20133, Milano, Italy}
\affil[24]{Institut d'Astrophysique de Paris, CNRS/Sorbonne Université, Paris, France}
\affil[25]{Max Planck Institute for Astrophysics, Karl-Schwarzschild-Str. 1, D-85748 Garching, Germany}
\affil[26]{Excellence Cluster ORIGINS, Boltzmannstr. 2, 85748 Garching, Germany}
\affil[27]{INFN Sezione di Roma2, Università di Roma Tor Vergata, via della Ricerca Scientifica, 1, 00133 Roma, Italy}
\affil[28]{Jodrell Bank Centre for Astrophysics, Alan Turing Building, Department of Physics and Astronomy, School of Natural Sciences, The University of Manchester, Oxford Road, Manchester M13 9PL, UK}
\affil[29]{University of California, Berkeley, Space Sciences Laboratory,  Berkeley, CA 94720, USA}
\affil[30]{Lawrence Berkeley National Laboratory (LBNL), Computational Cosmology Center, Berkeley, CA 94720, USA}
\affil[31]{Kavli Institute for the Physics and Mathematics of the Universe (Kavli IPMU, WPI), UTIAS, The University of Tokyo, Kashiwa, Chiba 277-8583, Japan}
\affil[32]{Centre Spatial de Liège, Université de Liège, Avenue du Pré-Aily, 4031 Angleur, Belgium}
\affil[33]{Dipartimento di Fisica, Università La Sapienza, P. le A. Moro 2, Roma, Italy}
\affil[34]{INFN Sezione di Roma, P.le A. Moro 2, 00185 Roma, Italy}
\affil[35]{Institute of Particle and Nuclear Studies (IPNS), High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki 305-0801, Japan}
\affil[36]{CNRS-UCB International Research Laboratory, Centre Pierre Binétruy, UMI2007, Berkeley, CA 94720, USA}
\affil[37]{Dpto. de Física Moderna, Universidad de Cantabria, Avda. los Castros s/n, E-39005 Santander, Spain}
\affil[38]{INFN Sezione Milano Bicocca, Piazza della Scienza, 3, 20126 Milano, Italy}
\affil[39]{Istituto Nazionale di Fisica Nucleare–Laboratori Nazionali di Frascati (INFN–LNF), Via E. Fermi 40, 00044, Frascati, Italy}
\affil[40]{INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy}
\affil[41]{Instituto de Astrofísica de Canarias, E-38200 La Laguna, Tenerife, Canary Islands, Spain}
\affil[42]{McGill University, Physics Department, Montreal, QC H3A 0G4, Canada}
\affil[43]{Japan Aerospace Exploration Agency (JAXA), Institute of Space and Astronautical Science (ISAS), Sagamihara, Kanagawa 252-5210, Japan}
\affil[44]{The Graduate University for Advanced Studies (SOKENDAI), Miura District, Kanagawa 240-0115, Hayama, Japan}
\affil[45]{Université de Paris, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\affil[46]{NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
\affil[47]{Lawrence Berkeley National Laboratory (LBNL), Physics Division, Berkeley, CA 94720, USA}
\affil[48]{University of Milano Bicocca, Physics Department, p.zza della Scienza, 3, 20126 Milan, Italy}
\affil[49]{Departamento de Astrofísica, Universidad de La Laguna (ULL), E-38206, La Laguna, Tenerife, Spain}
\affil[50]{School of Physics and Astronomy, Cardiff University, Cardiff CF24 3AA, UK}
\affil[51]{INFN Sezione di Bologna, Viale C. Berti Pichat, 6/2 – 40127 Bologna, Italy}
\affil[52]{Center for Astrophysics and Space Astronomy, University of Colorado, Boulder, CO 80309, USA}
\affil[53]{Université Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\affil[54]{Department of Physics and Astronomy, University of British Columbia, 6224 Agricultural Road, Vancouver, BC V6T1Z1, Canada}
\affil[55]{David A. Dunlap Department of Astronomy and Astrophysics, 50 St. George Street, Toronto, ON M5S3H4, Canada}
\affil[56]{School of Physics and Astronomy, University of Minnesota, 115 Union St SE, Minneapolis, MN 55455, USA}
\affil[57]{Nagoya University, Kobayashi-Masukawa Institute for the Origin of Particle and the Universe, Aichi 464-8602, Japan}
\affil[58]{Okayama University, Department of Physics, Okayama 700-8530, Japan}
\affil[59]{Institute for Photon Science and Technology, The University of Tokyo, 7-3-1 Hongo, Bunkyo-ku, Tokyo 113-0033, Japan}
\affil[60]{Space Science Data Center, Italian Space Agency, via del Politecnico, 00133, Roma, Italy}
\affil[61]{Université Grenoble Alpes, CNRS, LPSC-IN2P3, 53, avenue des Martyrs, 38000 Grenoble, France}
\affil[62]{Université Paris-Saclay, CNRS, Institut d’Astrophysique Spatiale, 91405, Orsay, France}
\affil[63]{Gran Sasso Science Institute (GSSI), Viale F. Crispi 7, I-67100, L’Aquila, Italy}
\affil[64]{Institute of Astrophysics, Foundation for Research and Technology – Hellas, Vasilika Vouton, GR-70013 Heraklion, Greece}
\affil[65]{Department of Physics and ITCP, University of Crete, GR-70013, Heraklion, Greece}
\affil[66]{Suwa University of Science, Chino, Nagano 391-0292, Japan}
\affil[67]{Physics and Astronomy Dept., University College London (UCL), UK}
\affil[68]{The University of Tokyo, Department of Astronomy, Tokyo 113-0033, Japan}
\affil[69]{Dipartimento di Fisica, Università di Pisa, Largo B. Pontecorvo 3, 56127 Pisa, Italy}
\affil[70]{SLAC National Accelerator Laboratory, Kavli Institute for Particle Astrophysics and Cosmology (KIPAC),  Menlo Park, CA 94025, USA}
\affil[71]{Stanford University, Department of Physics,  CA 94305-4060, USA}
\affil[72]{Mullard Space Science Laboratory, University College London, London, UK}
\affil[73]{INAF – Astronomical Observatory of Trieste, Via G. B. Tiepolo 11, 34143 Trieste, Italy}

